Subspace Alignment Chains and the Degrees of Freedom of the Three-User MIMO Interference Channel

We show that the 3 user M_T x M_R MIMO interference channel has d(M,N)=min(M/(2-1/k),N/(2+1/k)) degrees of freedom (DoF) normalized by time, frequency, and space dimensions, where M=min(M_T,M_R), N=max(M_T,M_R), k=ceil{M/(N-M)}. While the DoF outer bound is established for every M_T, M_R value, the achievability is established in general subject to normalization with respect to spatial-extensions. Given spatial-extensions, the achievability relies only on linear beamforming based interference alignment schemes with no need for time/frequency extensions. In the absence of spatial extensions, we show through examples how essentially the same scheme may be applied over time/frequency extensions. The central new insight to emerge from this work is the notion of subspace alignment chains as DoF bottlenecks. The DoF value d(M,N) is a piecewise linear function of M,N, with either M or N being the bottleneck within each linear segment. The corner points of these piecewise linear segments correspond to A={1/2,2/3,3/4,...} and B={1/3,3/5,5/7,...}. The set A contains all values of M/N and only those for which there is redundancy in both M and N. The set B contains all values of M/N and only those for which there is no redundancy in either M or N. Our results settle the feasibility of linear interference alignment, introduced by Cenk et al., for the 3 user M_T x M_R MIMO interference channel, completely for all values of M_T, M_R. Specifically, the linear interference alignment problem (M_T x M_R, d)^3 (as defined in previous work by Cenk et al.) is feasible if and only if d<=floor{d(M,N)}. With and only with the exception of the values M/N\in B, we show that for every M/N value there are proper systems that are not feasible. Our results show that M/N\in A are the only values for which there is no DoF benefit of joint processing among co-located antennas at the transmitters or receivers.

==> arxivabstract.tex <==
We show that the 3 user $M_T\times M_R$ MIMO interference channel
where each transmitter is equipped with $M_T$ antennas and each
receiver is equipped with $M_R$ antennas  has $d(M,N) \define
\min\left(\frac{M}{2-1/\kappa}, \frac{N}{2+1/\kappa}\right)$ degrees
of freedom (DoF) normalized by time, frequency, \emph{and space}
dimensions, where  $M\define\min(M_T,M_R), N\define\max(M_T,M_R),
\kappa \define \lceil\frac{M}{N-M}\rceil$.  While the DoF outer
bound of $d(M,N)$ is established for every $M_T, M_R$ value, the
achievability of $d(M,N)$ DoF is established \emph{in general}
subject to a normalization with respect to spatial-extensions, i.e.,
the scaling of the number of antennas at all nodes.  The central new insight to emerge from this work is the
notion of subspace alignment chains as DoF bottlenecks. 


The DoF value $d(M,N)$ is a piecewise linear function of $M,N$, with
either $M$ or $N$ being the bottleneck within each linear segment
while the other value contains some redundancy, i.e., it can be
reduced without reducing the DoF. The corner points of these
piecewise linear segments correspond to two sets,
$\mathcal{A}\define\{1/2, 2/3, 3/4, \cdots\}$ and
$\mathcal{B}\define\{1/3,3/5,5/7,\cdots\}$. The set $A$ contains all
those values of $M/N$ and only those values of $M/N$ for which there
is redundancy in \emph{both} $M$ and $N$, i.e., either can be
reduced without reducing DoF. The set $\mathcal{B}$ contains all
those values of $M/N$ and only those values of $M/N$ for which there
is \emph{no redundancy} in {either} $M$ or $N$, i.e., neither can be
reduced without reducing DoF. 


Our results settle the question of feasibility of linear
interference alignment, introduced previously by Cenk et al.,  for
the $3$ user $M_T\times M_R$ MIMO interference channel, completely
for all values of $M_T,M_R$. Specifically, we show that the linear
interference alignment problem $(M_T\times M_R, d)^3$  is feasible if and only if $d\leq
\lfloor d(M,N)\rfloor$. With the exception of the values
$M/N\in\mathcal{B}$, and only with that exception, we show that for
every $M/N$ value there are proper systems that are not feasible.  


Our results show that  $M/N\in\mathcal{A}$ are the only values  for which
there is no DoF benefit of joint processing among co-located
antennas at the transmitters or receivers. This may also be seen as
a consequence of the maximum redundancy in the $M/N\in\mathcal{A}$
settings.

